Combinatorial Rising Bandits

Combinatorial online learning is a fundamental task for selecting the optimal action (or super arm) as a combination of base arms in sequential interactions with systems providing stochastic rewards. It is applicable to diverse domains such as robotics, social advertising, network routing, and recommendation systems. In many real-world scenarios, we often encounter rising rewards, where playing a base arm not only provides an instantaneous reward but also contributes to the enhancement of future rewards, e.g., robots improving through practice and social influence strengthening in the history of successful recommendations. Crucially, these enhancements may propagate to multiple super arms that share the same base arms, introducing dependencies beyond the scope of existing bandit models. To address this gap, we introduce the Combinatorial Rising Bandit (CRB) framework and propose a provably efficient and empirically effective algorithm, Combinatorial Rising Upper Confidence Bound (CRUCB). We empirically demonstrate the effectiveness of CRUCB in realistic deep reinforcement learning environments and synthetic settings, while our theoretical analysis establishes tight regret bounds. Together, they underscore the practical impact and theoretical rigor of our approach. Our code is available at https://github.com/ml-postech/Combinatorial-Rising-Bandits.

==> figure/tex/ICLR_deeprl_env.tex <==
\begin{wrapfigure}{r}{0.4\linewidth}
\vspace{-0.8cm}
% \vspace{-6pt}
    \centering
    \begin{subfigure}{\linewidth}
        \centering
        % \includegraphics[width=0.85\linewidth,  trim={0.2cm 0 0.2cm 0}, clip]{./figure/images/AntMaze_easy2.png}
        \includegraphics[width=1\linewidth,  trim={0.2cm 0 0.2cm 0}, clip]{./figure/images/path_ant_easy.pdf}
        % \vspace{0.1cm}
        \caption{AntMaze-easy}
        \label{figure:antmaze-easy}
    \end{subfigure}
    \vfill
    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=0.8\linewidth]{./figure/images/path_ant_complex.pdf}
        % \includegraphics[width=\linewidth]{./figure/images/AntMaze_complex2.pdf}
        % \vspace{0.1cm}
        \caption{AntMaze-complex}
        \label{figure:antmaze-complex}
    \end{subfigure}
    \vspace{-0.4cm}
    \caption{\textbf{Deep RL environments.}
    An ant robot navigates the shortest path from start to goal via intermediate nodes, encountering three types of edges in (a):
\textcolor[HTML]{FF0000}{impossible edge} ($e_1$), \textcolor[HTML]{FF8C00}{bottleneck edge} ($e_3$), and \textcolor[HTML]{008000}{wide edge} ($e_2, e_4, e_5, e_6, e_7$).
    (b) Focus on \textcolor[HTML]{FF0000}{impossible edges} and \textcolor[HTML]{008000}{wide edges} in a complex map.
    }
    \label{figure:deeprl_environments}
    \vspace{-0.7cm}
\end{wrapfigure}


==> figure/tex/ICLR_heatmap.tex <==
\begin{wrapfigure}{r}{0.4\linewidth}
\centering
\vspace{-0.5cm}
    \begin{subfigure}{1.0\linewidth}
    \centering
        \includegraphics[width=\linewidth]{./figure/images/colorbar1.pdf}
    \end{subfigure}
    \vspace{-0.1cm}
    \centering
    \begin{subfigure}{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={3.2cm 1cm 3.2cm 1cm},clip]{./figure/images/heatmap3_oracle_3000.pdf}
        \caption{optimal policy}
        \label{figure:heatmap_Oracle}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={3.2cm 1cm 3.2cm 1cm},clip]{./figure/images/heatmap3_RCUCB_3000.pdf}
        \caption{CRUCB}
        \label{figure:heatmap-RCUCB}
    \end{subfigure}
    \vfill
    \begin{subfigure}{0.48\linewidth}
        \centering
       \includegraphics[width=\linewidth, trim={3.2cm 1cm 3.2cm 1cm},clip]{./figure/images/heatmap3_RUCB_3000.pdf}
        \caption{R-ed-UCB}
        \label{figure:heatmap_R-ed-UCB}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\linewidth}
        \centering
       \includegraphics[width=\linewidth, trim={3.2cm 1cm 3.2cm 1cm},clip]{./figure/images/heatmap3_SWCUCB_3000.pdf}
        \caption{SW-CUCB}
        \label{figure:heatmap_SWCUCB}
    \end{subfigure}
    
    \vspace{-0.1cm}
    \caption{\textbf{Heatmap of visit frequencies in AntMaze-complex.} 
    We visualize the visit frequencies for 
    the optimal policy, 
    CRUCB, R-ed-UCB
    , and SW-CUCB 
    highlighting the exploration patterns without prior knowledge of the environment.
    Visualizations for the other baselines are in Appendix~\ref{sec:heatmap}.
    }
    \label{figure:heatmap}
\end{wrapfigure}


==> figure/tex/ICLR_heatmap2.tex <==
\begin{wrapfigure}{r}{0.34\linewidth}
\centering
% \vspace{0.2cm}
    \begin{subfigure}{1.0\linewidth}
    \centering
        \includegraphics[width=\linewidth]{./figure/images/colorbar1.pdf}
    \end{subfigure}
    \vspace{-0.1cm}
    \centering
    \begin{subfigure}{0.06\linewidth}
        \rotatebox{90}{$t$ = 100}
        \vspace{0.6cm}
        \vfill
        \rotatebox{90}{$t$ = 3000}
        \vspace{0.6cm}
    \end{subfigure}
    \begin{subfigure}{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={3.2cm 1cm 3.2cm 1cm},clip]{./figure/images/heatmap3_RCUCB_100.pdf}
        \includegraphics[width=\linewidth, trim={3.2cm 1cm 3.2cm 1cm},clip]{./figure/images/heatmap3_RCUCB_3000.pdf}
        \caption{CRUCB}
        \label{figure:heatmap_RCUCB}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={3.2cm 1cm 3.2cm 1cm},clip]{./figure/images/heatmap3_RUCB_100.pdf}
        \includegraphics[width=\linewidth, trim={3.2cm 1cm 3.2cm 1cm},clip]{./figure/images/heatmap3_RUCB_3000.pdf}
        \caption{R-ed-UCB}
        \label{figure:heatmap_R-ed-UCB}
    \end{subfigure}
    \caption{\textbf{Heatmap of visit frequencies in AntMaze-complex.} 
        We visualize the visit frequencies of CRUCB and R-ed-UCB at time steps 100 and 3000 to highlight their respective exploration patterns. 
        Visualizations of other baselines are provided in Appendix~\ref{sec:heatmap}.}
    \label{figure:heatmap}
    \vspace{-0.5cm}
\end{wrapfigure}


==> figure/tex/ICLR_heatmap3.tex <==
\begin{wrapfigure}{r}{0.48\linewidth}  % 폭을 넓혀 글자 선명도 확보
\centering
\vspace{-0.5cm}
\includegraphics[width=0.9\linewidth]{./figure/images/colorbar3.pdf}
% \vspace{2pt}

% --- time labels (좌측) ---
\begin{subfigure}{0.08\linewidth}
  \centering
  \rotatebox{90}{$t=500$}
  \vspace{0.6cm}
  \vfill
  \rotatebox{90}{$t=3000$}
  \vspace{0.6cm}
\end{subfigure}
\hspace{-0.2cm}
% --- (a) CRUCB ---
\begin{subfigure}{0.28\linewidth}
  \centering
  \includegraphics[width=\linewidth,trim={3.2cm 1cm 3.2cm 1cm},clip]{./figure/images/heatmap7_CSWUCB_500-n.pdf}
  \includegraphics[width=\linewidth,trim={3.2cm 1cm 3.2cm 1cm},clip]{./figure/images/heatmap7_CSWUCB_3000-n.pdf}
  \caption{SW-CUCB}
  \label{figure:heatmap-SWCUCB}
\end{subfigure}
\hfill
% --- (b) R-ed-UCB ---
\begin{subfigure}{0.28\linewidth}
  \centering
  \includegraphics[width=\linewidth,trim={3.2cm 1cm 3.2cm 1cm},clip]{./figure/images/heatmap7_RUCB_500-n.pdf}
  \includegraphics[width=\linewidth,trim={3.2cm 1cm 3.2cm 1cm},clip]{./figure/images/heatmap7_RUCB_3000-n.pdf}
  \caption{R-ed-UCB}
  \label{figure:heatmap-RUCB} 
\end{subfigure}
\hfill
% --- (c) SW-CUCB ---
\begin{subfigure}{0.28\linewidth}
  \centering
  \includegraphics[width=\linewidth,trim={3.2cm 1cm 3.2cm 1cm},clip]{./figure/images/heatmap7_RCUCB_500-n.pdf}
  \includegraphics[width=\linewidth,trim={3.2cm 1cm 3.2cm 1cm},clip]{./figure/images/heatmap7_RCUCB_3000-n.pdf}
  \caption{CRUCB}
  \label{figure:heatmap-CRUCB}
\end{subfigure}
\captionsetup{skip=2pt}
\caption{\textbf{Heatmap of visit frequencies in AntMaze-complex.}
 We visualize the visit frequencies of SW-CUCB, R-ed-UCB, and CRUCB at time steps 500 and 3000 to highlight their respective exploration patterns.  Visualizations of other baselines are provided in Appendix~\ref{sec:heatmap}.}
\label{figure:heatmap}
\vspace{-0.3cm}
\end{wrapfigure}


==> figure/tex/constraint_bound_gap.tex <==
\begin{figure*}[!t]
    \centering
    \begin{subfigure}{0.45\linewidth}
        \centering
        \includegraphics[width=0.9\linewidth]{./figure/images/c.pdf}
        \caption{Reward function constraint.}
        \label{figure:constraint}
    \end{subfigure}
    \hspace{1cm}
    \begin{subfigure}{0.45\linewidth}
        \centering
        \includegraphics[width=0.9\linewidth] {./figure/images/bound_gap.pdf}
        \caption{Regret bound gap.}
        \label{figure:bound_gap}
    \end{subfigure}
    \vspace{-0.1cm}
    \caption{
    \textbf{Regret upper and lower bounds under the reward function growth under the $(n+1)^{-c}$ constraint.} This figure shows how $\mu_i(n)$ changes, where $\gamma_i(n) = C (n+1)^{-c}$, and $C$ is a normalized constant chosen such that $\mu(T) = 1$ when $\mu(0) = 0$. Smaller values of $c$ require more time steps to reach the maximum, leading to more samples needed to assess each base arm's potential, while larger $c$ values result in quicker judgments.
    }
    \label{figure:constraint_bound_gap}
    \vspace{-0.3cm}
\end{figure*}

==> figure/tex/deeprl_reward_env.tex <==
\begin{figure*}[!ht]
    \centering
    \begin{subfigure}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={1cm 0 1cm 0.8cm},clip]{./figure/images/reward_AntMaze-easy-n.pdf}
        \vspace{-0.7cm}
        \caption{Observed outcomes}
        \label{figure:reward-easy}
    \end{subfigure}
    \hspace{0.7cm}
    \begin{subfigure}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figure/images/AntMaze_easy2.png}
        % \vspace{0.1cm}
        \caption{AntMaze-easy}
        \label{figure:antmaze-easy}
    \end{subfigure}
    \hspace{0.3cm}
    \begin{subfigure}{0.3\linewidth}
        \centering
        \includegraphics[width=0.7\linewidth]{./figure/images/AntMaze_complex2.png}
        % \includegraphics[width=\linewidth]{./figure/images/AntMaze_complex2.pdf}
        % \vspace{0.1cm}
        \caption{AntMaze-complex}
        \label{figure:antmaze-complex}
    \end{subfigure}
    \vspace{-0.3cm}
    \caption{\textbf{Deep RL environments.}
    (a) Observed outcomes for each edge in (b).
    An ant robot navigates the shortest path from start to goal via intermediate nodes, encountering three types of edges in (b):
    impossible edge ($e_1$), late bloomer ($e_3$), and early peakers ($e_2, e_4, e_5, e_6, e_7$).
    (c) Focus on impossible edges and early peakers in a large map.
    }
    \label{figure:deeprl_environments}
    \vspace{-0.15cm}
\end{figure*}

==> figure/tex/deeprlenvironment.tex <==
\begin{figure}[!t]
    \centering
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figure/images/AntMaze_easy2.pdf}
        \caption{AntMaze-easy}
        \label{figure:antmaze-easy}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{./figure/images/AntMaze_complex2.pdf}
        \caption{AntMaze-complex}
        \label{figure:antmaze-complex}
    \end{subfigure}
    \vspace{-0.1cm}
    \caption{\textbf{Deep reinforcement learning environments}.
    We evaluate CRUCB and the baselines in the MuJoCo environments illustrated above,
    where the ant robot starts from the initial state. Intermediate nodes for path planning are represented by blue squares, and the goal node is marked by a red square.
    We note that the agent does not have access to the maps of the environments.
    }
    \label{figure:deeprl_environments}
    % \vspace{-0.3cm}
\end{figure}

==> figure/tex/deeprlregret.tex <==
\begin{figure}[!h]
    \centering
    \begin{subfigure}{0.9\linewidth}
    \centering
        \includegraphics[width=\linewidth]{./figure/images/legend3_1.pdf}
    \end{subfigure}
    \vfill
    \centering
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={1cm 0 1cm 0.8cm},clip]{./figure/images/regret_AntMaze-easy_2000_1.pdf}
        \vspace{-0.7cm}
        \caption{AntMaze-easy}
        \label{figure:regret_antmaze-easy}
    \end{subfigure}
    \hspace{1cm}
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={1cm 0 1cm 0.8cm},clip]{./figure/images/regret_AntMaze-complex_3000_1.pdf}
        \vspace{-0.7cm}
        \caption{AntMaze-complex}
        \label{figure:regret_antmaze-complex}
    \end{subfigure}
    % \hfill
    % \begin{subfigure}{0.32\linewidth}
    %     \centering
    %    \includegraphics[width=\linewidth]{regret_Reacher3D.pdf}
    %     \caption{Reacher3D}
    %     \label{figure:regret_reacher3D}
    % \end{subfigure}
    \vspace{-0.1cm}
    \caption{\textbf{Cumulative regret in deep reinforcement learning environments.}
    We report the average cumulative regret as a line and the 99\% confidence interval as a shaded region, based on 3 runs.}
    \label{figure:regret_deeprl}
\end{figure}

==> figure/tex/env_easy.tex <==
\begin{figure*}[!t]
    \centering
    \begin{subfigure}{0.28\linewidth}
        \centering
        \includegraphics[width=0.99\linewidth, trim={1cm 0 1cm 0.8cm},clip]{./figure/images/reward_simul_easy.pdf}
        \vspace{-0.7cm}
        \caption{rewards of each arm}
        \label{figure:reward_simul_simple}
    \end{subfigure}
    \hspace{1cm}
    \begin{subfigure}{0.23\linewidth}
        \centering
        \includegraphics[width=0.75\linewidth]{./figure/images/graph_Path_easy.png}
        \caption{graph structure}
        \label{figure:graph_path_simple}
    \end{subfigure}
    \hspace{1cm}
    \begin{subfigure}{0.26\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={1cm 0 1cm 0.8cm},clip]{./figure/images/regret2_Path_0.01_easy.pdf}
        \vspace{-0.7cm}
        \caption{regret}
        \label{figure:regret_shortest_path_simple}
    \end{subfigure}
    % \vspace{-0.2cm}
    \caption{\textbf{Cumulative regret for online shortest path task in simple environment.} 
    We report the average cumulative regret as a line and the 99\% confidence interval as a shaded region, based on 5 runs.}
    \label{figure:regret_easy_path}
    \vspace{-0.3cm}
\end{figure*}



==> figure/tex/environment.tex <==
\begin{figure*}[!t]
    \centering
    \begin{subfigure}{0.28\linewidth}
        \centering
        \includegraphics[width=0.99\linewidth, trim={1cm 0 1cm 0.8cm},clip]{./figure/images/reward_simul4.pdf}
        \vspace{-0.7cm}
        \caption{rewards of each arm}
        \label{figure:reward_simul}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.23\linewidth}
        \centering
        \includegraphics[width=0.75\linewidth]{./figure/images/graph_Path2.png}
        \caption{Online shortest path}
        \label{figure:graph_path}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=0.75\linewidth]{./figure/images/graph_Matching2.png}
        \caption{Maximum weighted matching}
        \label{figure:graph_matching}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.23\linewidth}
        \centering
        \includegraphics[width=0.75\linewidth]{./figure/images/graph_Spanning2.png}
        \caption{Minimum spanning tree}
        \label{figure:graph_spanning}
    \end{subfigure}
    % \vspace{-0.2cm}
    \caption{\textbf{Synthetic environments.}
    We evaluate CRUCB and the baselines in the set of synthetic environments depicted above. (a) Outcome graphs illustrating two types of edges: a late bloomer with initially low but rising outcomes, and an early peaker with initially high but non-rising outcomes. Graph structures used in each task are shown in (b) Online shortest path, (c) Maximum weighted matching, and (d) Minimum spanning tree.
    }
    \label{figure:environments}
    \vspace{-0.3cm}
\end{figure*}

==> figure/tex/environment_easy.tex <==
\begin{figure*}[!t]
    \centering
    \begin{subfigure}{0.25\linewidth}
        \centering
        \includegraphics[width=0.99\linewidth, trim={1cm 0 1cm 0.8cm},clip]{./figure/images/reward_easy.pdf}
        \vspace{-0.7cm}
        \caption{Outcome functions}
        \label{figure:reward_simul_easy}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.23\linewidth}
        \centering
        \includegraphics[width=0.75\linewidth]{./figure/images/graph_Path_easy.png}
        \caption{Online shortest path}
        \label{figure:graph_path_easy}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=0.75\linewidth]{./figure/images/graph_Matching_easy.png}
        \caption{Maximum weighted matching}
        \label{figure:graph_matching_easy}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.23\linewidth}
        \centering
        \includegraphics[width=0.75\linewidth]{./figure/images/graph_Spanning_easy.png}
        \caption{Minimum spanning tree}
        \label{figure:graph_spanning_easy}
    \end{subfigure}
    % \vspace{-0.2cm}
    \caption{\textbf{Simple synthetic environments.}
    (a) Outcome graph.
    Graph structures used in each task are shown in (b) Online shortest path, (c) Maximum weighted matching, and (d) Minimum spanning tree.
    }
    \label{figure:environments_easy}
    \vspace{-0.3cm}
\end{figure*}

==> figure/tex/heatmap.tex <==
\begin{figure}[!ht]
\centering
    \begin{subfigure}{0.6\linewidth}
    \centering
        \includegraphics[width=\linewidth]{./figure/images/colorbar1.pdf}
    \end{subfigure}
    \vspace{-0.1cm}
    \vfill
    \centering
    \begin{subfigure}{0.22\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={3.2cm 1cm 3.2cm 1cm},clip]{./figure/images/heatmap3_oracle_3000.pdf}
        \caption{optimal policy}
        \label{figure:heatmap_Oracle}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.22\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={3.2cm 1cm 3.2cm 1cm},clip]{./figure/images/heatmap3_RCUCB_3000.pdf}
        \caption{CRUCB (Ours)}
        \label{figure:heatmap-RCUCB}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.22\linewidth}
        \centering
       \includegraphics[width=\linewidth, trim={3.2cm 1cm 3.2cm 1cm},clip]{./figure/images/heatmap3_RUCB_3000.pdf}
        \caption{R-ed-UCB}
        \label{figure:heatmap_R-ed-UCB}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.22\linewidth}
        \centering
       \includegraphics[width=\linewidth, trim={3.2cm 1cm 3.2cm 1cm},clip]{./figure/images/heatmap3_SWCUCB_3000.pdf}
        \caption{SW-CUCB}
        \label{figure:heatmap_SWCUCB}
    \end{subfigure}
    \vspace{-0.1cm}
    \caption{\textbf{Heatmap of visit frequencies in AntMaze-complex.} 
    We visualize the visit frequencies for the optimal policy, CRUCB, R-ed-UCB, and SW-CUCB, highlighting the exploration patterns without prior knowledge of the environment.
    Visualizations for the other baselines are in Appendix~\ref{sec:heatmap}.
    }
    \label{figure:heatmap}
\end{figure}


==> figure/tex/icml_simul_path.tex <==
\begin{figure*}[!h]
    \centering
    \begin{subfigure}{0.8\linewidth}
    \centering
        \includegraphics[width=\linewidth]{./figure/images/legend3_1.pdf}
    \end{subfigure}
    \vfill
    \begin{subfigure}{0.28\linewidth}
        \centering
        \includegraphics[width=0.75\linewidth]{./figure/images/graph_path_complex.png}
        \caption{Graph structure}
        \label{figure:graph_path}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=0.95\linewidth, trim={1cm 0 1cm 0.8cm},clip]{./figure/images/reward_complex.pdf}
        \vspace{-0.3cm}
        \caption{Outcome functions}
        \label{figure:reward}
    \end{subfigure}
    \hfill
    % \begin{subfigure}{0.26\linewidth}
    %     \centering
    %     \includegraphics[width=0.99\linewidth, trim={1cm 0 1cm 0.8cm},clip]{./figure/images/regret_path_short.pdf}
    %     \vspace{-0.7cm}
    %     \caption{Cumulative regret (50K)}
    %     \label{figure:regret_path_short}
    % \end{subfigure}
    % \hfill
    \begin{subfigure}{0.34\linewidth}
        \centering
        \includegraphics[width=0.99\linewidth, trim={1cm 0 1cm 0.8cm},clip]{./figure/images/regret_path_full.pdf}
        \vspace{-0.7cm}
        \caption{Cumulative regret}
        \label{figure:regret_path_full}
    \end{subfigure}
    
    \caption{\textbf{Online shortest path planning task.}
        We evaluate CRUCB and the baselines in the online shortest path planning task on the graph structure depicted above.
        (a) Simple graph structure.
        (b) Outcome graph for the simple graph structure, illustrating two types of edges: a late bloomer $(c=1.2)$ with initially low but rising outcomes, and an early peaker with initially high but non-rising outcomes.
        There are two vertical lines: the \textcolor[HTML]{1E90FF}{first line} represents the point where the rewards of the late bloomer and early peaker become equal, and the \textcolor[HTML]{8A2BE2}{second line} represents the point where the sum of their cumulative rewards becomes equal.
        % (c) Zoomed-in view of the cumulative regret, focusing on the initial part.
        (c) Cumulative regret.
        We report the average cumulative regret as a line and the 99\% confidence interval as a shaded region, based on 5 runs.
    }
    \label{figure:path}
    \vspace{-0.3cm}
\end{figure*}


==> figure/tex/icml_simul_path_easy.tex <==
\begin{figure*}[!t]
    \centering
    \begin{subfigure}{0.8\linewidth}
    \centering
        \includegraphics[width=\linewidth]{./figure/images/legend3_1.pdf}
    \end{subfigure}
    \vfill
    \begin{subfigure}{0.2\linewidth}
        \centering
        \includegraphics[width=0.75\linewidth]{./figure/images/graph_Path_easy.png}
        \caption{Simple graph structure}
        \label{figure:graph_path_simple}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.27\linewidth}
        \centering
        \includegraphics[width=0.95\linewidth, trim={1cm 0 1cm 0.8cm},clip]{./figure/images/icml_reward_simul_easy.pdf}
        \vspace{-0.3cm}
        \caption{Simple graph reward functions}
        \label{figure:reward_path_simple}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.25\linewidth}
        \centering
        \includegraphics[width=0.99\linewidth, trim={1cm 0 1cm 0.8cm},clip]{./figure/images/icml_short_regret_simul_path_easy.pdf}
        \vspace{-0.7cm}
        \caption{Cumulative regret}
        \label{figure:short_regret_path_simple}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.25\linewidth}
        \centering
        \includegraphics[width=0.99\linewidth, trim={1cm 0 1cm 0.8cm},clip]{./figure/images/icml_regret_simul_path_easy.pdf}
        \vspace{-0.7cm}
        \caption{Cumulative regret (full)}
        \label{figure:regret_path_simple}
    \end{subfigure}
    
    \caption{\textbf{Online shortest path planning task for simple graph structure.}
        We evaluate CRUCB and the baselines in the online shortest path planning task on the graph structure depicted above.
        (a) Simple graph structure.
        (b) Outcome graph for the simple graph structure, illustrating two types of edges: a late bloomer with initially low but rising outcomes, and an early peaker with initially high but non-rising outcomes.
        There are two vertical lines: the first line represents the point where the rewards of the late bloomer and early peaker become equal, and the second line represents the point where the sum of their cumulative rewards becomes equal.
        (c, d) Cumulative regret.
    }
    \label{figure:path_simple}
    \vspace{-0.3cm}
\end{figure*}



==> figure/tex/othertask.tex <==
\begin{figure*}[!t]
    \centering
    \begin{subfigure}{0.25\linewidth}
        \centering
        \includegraphics[width=0.99\linewidth, trim={1cm 0 1cm 0.8cm},clip]{./figure/images/reward_complex.pdf}
        \vspace{-0.7cm}
        \caption{Outcome functions}
        \label{figure:reward_app}
    \end{subfigure}
    \hspace{1cm}
    \begin{subfigure}{0.24\linewidth}
        \centering
        \includegraphics[width=0.75\linewidth]{./figure/images/graph_Matching2.png}
        \caption{Maximum weighted matching}
        \label{figure:graph_matching}
    \end{subfigure}
    \hspace{1cm}
    \begin{subfigure}{0.23\linewidth}
        \centering
        \includegraphics[width=0.75\linewidth]{./figure/images/graph_Spanning2.png}
        \caption{Minimum spanning tree}
        \label{figure:graph_spanning}
    \end{subfigure}
    % \vspace{-0.2cm}
    \caption{\textbf{Synthetic environments for Maximum weighted matching and Minimum spanning tree tasks.}
    (a) Outcome graph.
    Graph structures used in each task are shown in (b) Maximum weighted matching, and (c) Minimum spanning tree.
    }
    \label{figure:othertask}
    \vspace{-0.3cm}
\end{figure*}

==> figure/tex/path_planning.tex <==
\begin{figure*}[!t]
    \centering
    
    \begin{subfigure}{0.2\linewidth}
        \centering
        \includegraphics[width=0.75\linewidth]{./figure/images/graph_Path_easy.png}
        \caption{Simple graph structure}
        \label{figure:graph_path_simple}
    \end{subfigure}
    \hspace{0.1cm}
    \begin{subfigure}{0.27\linewidth}
        \centering
        \includegraphics[width=0.99\linewidth, trim={1cm 0 1cm 0.8cm},clip]{./figure/images/reward_simul_easy.pdf}
        \vspace{-0.7cm}
        \caption{Simple graph reward functions}
        \label{figure:reward_simul_simple}
    \end{subfigure}
    \hspace{0.1cm}
    \begin{subfigure}{0.21\linewidth}
        \centering
        \includegraphics[width=0.75\linewidth]{./figure/images/graph_Path2.png}
        \caption{Complex graph structure}
        \label{figure:graph_path}
    \end{subfigure}
    \hspace{0.1cm}
    \begin{subfigure}{0.27\linewidth}
        \centering
        \includegraphics[width=0.99\linewidth, trim={1cm 0 1cm 0.8cm},clip]{./figure/images/reward_simul4.pdf}
        \vspace{-0.7cm}
        \caption{Complex graph reward functions}
        \label{figure:reward_simul}
    \end{subfigure}
    \caption{\textbf{Online shortest path planning task.}
        We evaluate CRUCB and the baselines in the online shortest path planning task on the graph structures depicted above.
        (a) Simple graph structure.
        (b) Outcome graph for the simple graph structure, illustrating two types of edges: a late bloomer with initially low but rising outcomes, and an early peaker with initially high but non-rising outcomes.
        (c) Complex graph structure.
        (d) Outcome graph for the complex graph structure.
    }
    \label{figure:env_path}
    \vspace{-0.3cm}
\end{figure*}



==> figure/tex/regret.tex <==
\begin{figure*}[!t]
    \centering
    \begin{subfigure}{0.7\linewidth}
    \centering
        \includegraphics[width=\linewidth]{./figure/images/legend3_1.pdf}
    \end{subfigure}
    \vfill
    \centering
    \begin{subfigure}{0.26\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={1cm 0 1cm 0.8cm},clip]{./figure/images/regret2_Path_0.01.pdf}
        \vspace{-0.7cm}
        \caption{Online shortest path}
        \label{figure:regret_shortest_path}
    \end{subfigure}
    \hspace{1cm}
    \begin{subfigure}{0.26\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={1cm 0 1cm 0.8cm},clip]{./figure/images/regret2_Matching_0.01.pdf}
        \vspace{-0.7cm}
        \caption{Maximum weighted matching}
        \label{figure:regret_matching}
    \end{subfigure}
    \hspace{1cm}
    \begin{subfigure}{0.26\linewidth}
        \centering
       \includegraphics[width=\linewidth, trim={1cm 0 1cm 0.8cm},clip]{./figure/images/regret2_Spanning_0.01.pdf}
       \vspace{-0.7cm}
        \caption{Minimum spanning tree}
        \label{figure:regret_spanning_Tree}
    \end{subfigure}
    % \vspace{-0.2cm}
    \caption{\textbf{Cumulative regret for each task in synthetic environments.} 
    We report the average cumulative regret as a line and the 99\% confidence interval as a shaded region, based on 5 runs.}
    \label{figure:regret}
    \vspace{-0.3cm}
\end{figure*}



==> figure/tex/regret_easy.tex <==
\begin{figure*}[!t]
    \centering
    \begin{subfigure}{0.7\linewidth}
    \centering
        \includegraphics[width=\linewidth]{./figure/images/legend3_1.pdf}
    \end{subfigure}
    \vfill
    \centering
    \begin{subfigure}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={1cm 0 1cm 0.8cm},clip]{./figure/images/regret_path_easy.pdf}
        \vspace{-0.7cm}
        \caption{Online shortest path}
        \label{figure:regret_path_easy}
    \end{subfigure}
    \hspace{0.5cm}
    \begin{subfigure}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={1cm 0 1cm 0.8cm},clip]{./figure/images/regret_matching_easy.pdf}
        \vspace{-0.7cm}
        \caption{Maximum weighted matching}
        \label{figure:regret_matching_easy}
    \end{subfigure}
    \hspace{0.5cm}
    \begin{subfigure}{0.3\linewidth}
        \centering
       \includegraphics[width=\linewidth, trim={1cm 0 1cm 0.8cm},clip]{./figure/images/regret_spanning_easy.pdf}
       \vspace{-0.7cm}
        \caption{Minimum spanning tree}
        \label{figure:regret_spanning_easy}
    \end{subfigure}
    % \vspace{-0.2cm}
    \caption{\textbf{Cumulative regret for each task in simple synthetic environments.} 
    We report the average cumulative regret as a line and the 99\% confidence interval as a shaded region, based on 5 runs.}
    \label{figure:regret_easy}
    \vspace{-0.3cm}
\end{figure*}



==> figure/tex/regret_gap.tex <==
  %\vspace{-0.8cm} % 위쪽 여백 줄이기
  %\centering
  % --- Left: Theorem ---
\begin{minipage}[c]{0.57\textwidth} % [c] for vertical centering

    \begin{theorem}[Regret lower bound over a \textbf{general} class] \label{thm:lower_bound}
        Fix sufficiently large time $T$.
        Let $\mathcal{I}$ be the set of all available CRB instances. 
        Then, any policy $\pi$ suffers regret:
        \[
            \min_{\pi}\max_{\nu\in\mathcal{I}}\textit{Reg}_{\nu}(\pi,T) = \Omega(LT)\;,
         \]
         where $L$ is the maximum size of super arms.
    \end{theorem}

    \vspace{0pt}
    \begin{theorem}[Regret lower bound over a fine-grained class] \label{thm:lower_bound_2}
      Fix sufficiently large $T$. For $1<c<2$, define $\mathcal{A}_c$ as follows:
      \[
        \mathcal{A}_c := \{\nu:\gamma_i(n)\le (n+1)^{-c},\, i\in[K],\, n\in[T-1]\}.
      \]
      Then
      \[
        \min_{\pi}\max_{\nu\in\mathcal{A}_c}\mathrm{Reg}_\nu(\pi,T)
        = \Omega\big(\!\max\{L\sqrt{T},\,LT^{2-c}\}\!\big),
      \]
      where $L := \max_{S\in\mathcal{S}}|S|$.
    \end{theorem}
  \end{minipage}
  \hfill
  % --- Right: Figure --- 
  \begin{minipage}[c]{0.40\textwidth} % [c] for vertical centering
  %\begin{figure}[t]
    \vspace{0pt}
    \centering
    \includegraphics[width=\linewidth]{figure/images/bound_gap.pdf}
    \captionof{figure}{\textbf{Visualization of regret bounds. %(Theorem~\ref{thm:lower_bound_2}).
    } 
  % For $f(n)=(n+1)^{-c}$, the CRB lower bound and the CRUCB upper bound are of similar order for $1<c<1.5$ (lower: $2-c$, upper: $1/c$),while both equal $1$ for $c\le 1$.
  % \textbf{Left}: Theoretical regret lower bound of CRB under $f(n)=(n+1)^{-c}$. 
  \textbf{Right}: The regret lower bound of CRB and the regret upper bound of CRUCB under $f(n)$ (\eqref{eq:non-linear2} in Corollary~\ref{cor:characterize}), which are of similar order for $1\!<\!c\!<\!1.5$ (lower bound: $2\!-\!c$, upper bound: $1/c$), and both equal $1$ when $c\!\leq\!1$.
}
\vspace{-0.2cm}
  \label{figure:bound_gap}
%\end{figure}
  \end{minipage}

%   \vspace{-0.2cm}  
%   \caption{\textbf{Visualization of regret bounds (Theorem~\ref{thm:lower_bound_2}).} 
%   % For $f(n)=(n+1)^{-c}$, the CRB lower bound and the CRUCB upper bound are of similar order for $1<c<1.5$ (lower: $2-c$, upper: $1/c$),while both equal $1$ for $c\le 1$.
%   \textbf{Left}: Theoretical regret lower bound of CRB under $f(n)=(n+1)^{-c}$. 
%   \textbf{Right}: The regret lower bound of CRB and the regret upper bound of CRUCB under $f(n)$ (\eqref{eq:non-linear2} in Corollary~\ref{cor:characterize}), which are of similar order for $1\!<\!c\!<\!1.5$ (lower bound: $2\!-\!c$, upper bound: $1/c$), and both equal $1$ when $c\!\leq\!1$.
% }




==> figure/tex/regret_othertask.tex <==
\begin{figure*}[!t]
    \centering
    \begin{subfigure}{0.7\linewidth}
    \centering
        \includegraphics[width=\linewidth]{./figure/images/legend3_1.pdf}
    \end{subfigure}
    \vfill
    \centering
    \begin{subfigure}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={1cm 0 1cm 0.8cm},clip]{./figure/images/regret_matching.pdf}
        \vspace{-0.7cm}
        \caption{Maximum weighted matching}
        \label{figure:regret_matching}
    \end{subfigure}
    \hspace{1cm}
    \begin{subfigure}{0.3\linewidth}
        \centering
       \includegraphics[width=\linewidth, trim={1cm 0 1cm 0.8cm},clip]{./figure/images/regret_spanning.pdf}
       \vspace{-0.7cm}
        \caption{Minimum spanning tree}
        \label{figure:regret_spanning}
    \end{subfigure}
    \caption{\textbf{Cumulative regret for each task.} 
    We report the average cumulative regret as a line and the 99\% confidence interval as a shaded region, based on 5 runs.}
    \label{figure:regret_othertask}
    \vspace{-0.3cm}
\end{figure*}



==> figure/tex/regret_path_planning.tex <==
\begin{figure}[!t]
    \centering
    \begin{subfigure}{1.0\linewidth}
    \centering
        \includegraphics[width=\linewidth]{./figure/images/legend3_1.pdf}
    \end{subfigure}
    \vfill
    \centering
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={1cm 0 1cm 0.8cm},clip]{./figure/images/regret2_Path_0.01_easy.pdf}
        \vspace{-0.7cm}
        \caption{Simple graph}
        \label{figure:regret_shortest_path_simple}
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={1cm 0 1cm 0.8cm},clip]{./figure/images/regret2_Path_0.01.pdf}
        \vspace{-0.7cm}
        \caption{Complex graph}
        \label{figure:regret_shortest_path}
    \end{subfigure}
    \vspace{-0.1cm}
    \caption{\textbf{Cumulative regret for online shortest path planning tasks in synthetic environments.} 
    We report the average cumulative regret as a line, with the 99\% confidence interval represented as a shaded region, based on 5 runs.}
    \label{figure:regret_path}
    \vspace{-0.3cm}
\end{figure}



==> figure/tex/reward_easy.tex <==
\begin{figure}[!t]
    \centering
    \begin{subfigure}{0.6\linewidth}
    \centering
        \includegraphics[width=\linewidth, trim={1cm 0 1cm 0.8cm},clip]{AAAI25/figure/images/reward_AntMaze-easy.pdf}
    \end{subfigure}
    \caption{\textbf{Reward in AntMaze-easy scenario.}
        sfdfs}
    \label{figure:reward_easy}
\end{figure}

==> figure/tex/toy.tex <==
\begin{figure}[!t]
    \centering
    \begin{subfigure}{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{AAAI25/figure/images/graph_ToyPath.png}
        \caption{Toy environment}
        \label{figure:graph_toy}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.53\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={1cm 0 1cm 0.8cm},clip]{NeurIPS/figure/images/reward_toy2.pdf}
        \vspace{-0.7cm}
        \caption{reward}
        \label{figure:reward_toy}
    \end{subfigure}
    \vfill
    \vspace{0.1cm}
    \begin{subfigure}{0.8\linewidth}
    \centering
        \includegraphics[width=\linewidth]{AAAI25/figure/images/legend2_2.pdf}
    \end{subfigure}
    \vspace{-0.1cm}
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={1cm 0 1cm 0.8cm},clip]{AAAI25/figure/images/regret_ToyPath2_10.pdf}
        \vspace{-0.7cm}
        \caption{cumulative regret}
        \label{figure:regret_toy}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth, trim={1cm 0 1cm 0.8cm},clip]{AAAI25/figure/images/sel_arm_ToyPath.pdf}
        \vspace{-0.7cm}
        \caption{($e_0$, $e_2$) selection counts}
        \label{figure:arm_sel_toy}
    \end{subfigure}
    \caption{\textbf{Necessity of considering combinatorial nature in rising bandit.}
    We compare the cumulative regrets of CRUCB (Ours) with state-of-the-art non-stationary combinatorial bandit and rising bandit algorithms in the combinatorial rising bandit setting for the online shortest path problem in a toy environment whose graph is illustrated in Figure~\ref{figure:graph_toy}. 
    The reward of each arm is illustrated in Figure~\ref{figure:reward_toy}.
    There are three edges: $e_0$, which is commonly used in both paths and consistently increases; $e_1$, which starts low initially but increases; and $e_2$, which starts high from the beginning.
    Figure~\ref{figure:regret_toy} reports the average cumulative regret as a line and the 99\% confidence interval as a shaded region, based on 5 runs, and Figure~\ref{figure:arm_sel_toy} present the count of the early peaker path ($e_0$, $e_2$) selection.
    }
    \label{figure:toy}
    \vspace{-0.3cm}
\end{figure}

==> table/related_works.tex <==
\begin{table*}[!t]
    \centering
    \caption{\textbf{Summary of related works}}
        \begin{tabular}{c c c}
        \toprule
        Paper & Reward dynamics & Problem setting \\
        \toprule
        \citet{wang2023combinatorial, wang2018thompson} & stationary & combinatorial \\
        \cmidrule(lr){1-3}
        \citet{chen2021combinatorial,combes2015combinatorial} & non-stationary & combinatorial \\
        \cmidrule(lr){1-3}
        \citet{metelli2022stochastic, xia2024llm}& rising & non-combinatorial\\
        \cmidrule(lr){1-3}
        Our work & rising & combinatorial \\
        \bottomrule
        \label{table:related_works}
    \end{tabular}
\end{table*}

==> table/related_works_combinatorial.tex <==
\begin{table*}[!t]
    \centering
    \caption{\textbf{Previous researches on combinatorial bandit}}
        \begin{tabular}{c c c c c}
        \midrule
        Reward dynamics & Paper & Reward assumption & Feedback & Reward function\\
        \midrule
        \multirow{3}{*}{staitionary} & \cite{chen2013combinatorial} & \_ & semi-bandit & general \\
        \cmidrule(lr){2-5}
        & \cite{kveton2015combinatorial} & \_ & cascading & non-linear \\
        \cmidrule(lr){2-5}
        & \cite{wang2023combinatorial} & \_ & max & non-linear \\
        \cmidrule(lr){1-5}
        \multirow{2}{*}{non-stationary} & \cite{combes2015combinatorial} & restless & full-bandit & linear \\
        \cmidrule(lr){2-5}
        & \cite{chen2021combinatorial} & restless & semi-bandit & general \\
        \cmidrule(lr){1-5}
        rising & Our work & rested & semi-bandit & linear \\
        \bottomrule
        \label{table:combinatorial}
    \end{tabular}
\end{table*}




==> table/related_works_non-stationary.tex <==


\begin{table*}[!t]
    \centering
    % \tiny
    %\scriptsize
    % \footnotesize
    %\small
    \caption{\textbf{Previous researches on non-stationary bandit}}
    \begin{tabular}{c c c c}
        \toprule
        Reward dynamics & Paper &  Reward assumption & Reward distribution \\
        \midrule
        \multirow{4}{*}{non-staitionary} & \cite{garivier2011upper}  & restless & general \\
        \cmidrule(lr){2-4}
        & \cite{besbes2014stochastic} & restless & general \\
        \cmidrule(lr){2-4}
        & \cite{cao2019nearly} & restless & general \\
        \cmidrule(lr){2-4}
        & \cite{trovo2020sliding} & restless & Bernoulli \\
        \cmidrule(lr){1-4}
        \multirow{4}{*}{rising} & \cite{heidari2016tight} & rested, restless & deterministic \\
        \cmidrule(lr){2-4}
        & \cite{metelli2022stochastic} & rested, restless & subgaussian\\
        \cmidrule(lr){2-4}
        & \cite{xia2024llm} & rested &  subgaussian\\
        \cmidrule(lr){2-4}
        &  Our work & rested & subgaussian\\

        \bottomrule
        
        \label{table:non-stationary}
    \end{tabular}
\end{table*}


% \begin{table*}[!t]
%     \centering

%     \caption{\textbf{Related works}}
%     \begin{tabular}{c c c}
%         \toprule
%         Paper & Reward dynamics &  Problem setting\\
%         \midrule
%         \multirow{4}{*}{non-staitionary} & \cite{garivier2011upper}  & restless & general \\
%         \cmidrule(lr){2-4}
%         & \cite{besbes2014stochastic} & restless & general \\
%         \cmidrule(lr){2-4}
%         & \cite{cao2019nearly} & restless & general \\
%         \cmidrule(lr){2-4}
%         & \cite{trovo2020sliding} & restless & Bernoulli \\
%         \cmidrule(lr){1-4}
%         \multirow{4}{*}{rising} & \cite{heidari2016tight} & rested, restless & deterministic \\
%         \cmidrule(lr){2-4}
%         & \cite{metelli2022stochastic} & rested, restless & subgaussian\\
%         \cmidrule(lr){2-4}
%         & \cite{xia2024llm} & rested &  subgaussian\\
%         \cmidrule(lr){2-4}
%         &  Our work & rested & subgaussian\\

%         \bottomrule
        
%         \label{table:non-stationary}
%     \end{tabular}
% \end{table*}


